HATS-31b Through HATS-35b: Five Transiting Hot Jupiters Discovered by the HATSouth Survey

We report the discovery of five new transiting hot Jupiter planets discovered by the HATSouth survey: HATS-31b through HATS-35b. These planets orbit moderately bright stars with V magnitudes within the range 11.9-14.4mag while the planets span a range of masses 0.88-1.22MJ, and have somewhat inflated radii between 1.23-1.64RJ.These planets can be classified as typical hot Jupiters, with HATS-31b and HATS-35b being moderately inflated gas giant planets with radii of $1.64 \pm 0.22$ RJ and 1.464+0.069-0.044RJ, respectively, that can be used to constrain inflation mechanisms. All five systems present a higher Bayesian evidence for a fixed circular orbit model than for an eccentric orbit. The orbital periods range from $1.8209993 \pm 0.0000016$ day for HATS-35b) to $3.377960 \pm 0.000012$ day for HATS-31b. Additionally, HATS-35b orbits a relatively young F star with an age of $2.13 \pm 0.51$ Gyr. We discuss the analysis to derive the properties of these systems and compare them in the context of the sample of well characterized transiting hot Jupiters known to date.

==> data/HATS566-004_rvtable.tex <==
HATS-31 & $ 7067.77200 $ & $    68.51 $ & $    29.00 $ & $   -8.0 $ & $   58.0 $ & $   0.861 $ & HARPS \\
HATS-31 & $ 7068.80731 $ & $  -111.49 $ & $    22.00 $ & $  138.0 $ & $   44.0 $ & $   0.167 $ & HARPS \\
HATS-31 & $ 7069.83756 $ & $     5.51 $ & $    35.00 $ & $   98.0 $ & $   66.0 $ & $   0.472 $ & HARPS \\
HATS-31 & $ 7070.78858 $ & $    89.51 $ & $    22.00 $ & $   64.0 $ & $   44.0 $ & $   0.754 $ & HARPS \\
HATS-31 & $ 7071.81170 $ & $   -38.49 $ & $    15.00 $ & $   34.0 $ & $   32.0 $ & $   0.057 $ & HARPS \\
HATS-31 & $ 7072.81373 $ & $   -87.49 $ & $    18.00 $ & $   46.0 $ & $   40.0 $ & $   0.353 $ & HARPS \\


==> data/HATS586-004_rvtable.tex <==
HATS-32 & $ 6857.88391 $ & $   -65.26 $ & $    11.00 $ & $   -2.0 $ & $   15.0 $ & $   0.373 $ & FEROS \\
HATS-32 & $ 6858.83608 $ & $   142.74 $ & $    11.00 $ & $   43.0 $ & $   16.0 $ & $   0.712 $ & FEROS \\
HATS-32 & $ 7183.82218 $ & $  -157.26 $ & $    23.00 $ & $  -13.0 $ & $   30.0 $ & $   0.256 $ & FEROS \\
HATS-32 & $ 7184.92441 $ & $    96.74 $ & $    16.00 $ & $   47.0 $ & $   22.0 $ & $   0.648 $ & FEROS \\
HATS-32 & $ 7186.82299 $ & $   -67.26 $ & $    20.00 $ & $   61.0 $ & $   26.0 $ & $   0.323 $ & FEROS \\
HATS-32 & $ 7187.92768 $ & $   119.74 $ & $    13.00 $ & $  -43.0 $ & $   18.0 $ & $   0.716 $ & FEROS \\
HATS-32 & $ 7189.81850 $ & $  -121.26 $ & $    13.00 $ & $  -22.0 $ & $   18.0 $ & $   0.388 $ & FEROS \\
HATS-32 & $ 7190.90671 $ & $   102.74 $ & $    13.00 $ & $  -18.0 $ & $   18.0 $ & $   0.775 $ & FEROS \\


==> data/HATS747-032_rvtable.tex <==
HATS-33 & $ 7109.90663 $ & $  -115.04 $ & $    11.00 $ & $   16.0 $ & $   18.0 $ & $   0.307 $ & Coralie \\
HATS-33 & $ 7118.90238 $ & $   150.99 $ & $     7.00 $ & $    1.0 $ & $   28.0 $ & $   0.835 $ & HARPS \\
HATS-33 & $ 7119.85968 $ & $  -166.01 $ & $     9.00 $ & $  -22.0 $ & $   38.0 $ & $   0.211 $ & HARPS \\
HATS-33 & $ 7120.89565 $ & $   120.99 $ & $     6.00 $ & $   -2.0 $ & $   24.0 $ & $   0.617 $ & HARPS \\
HATS-33 & $ 7150.22296 $ & $   -94.90 $ & $    12.00 $ & \nodata      & \nodata      & $   0.120 $ & CYCLOPS2 \\
HATS-33 & $ 7150.23892 $ & $  -138.80 $ & $    12.40 $ & \nodata      & \nodata      & $   0.126 $ & CYCLOPS2 \\
HATS-33 & $ 7150.25487 $ & $  -101.70 $ & $    12.60 $ & \nodata      & \nodata      & $   0.133 $ & CYCLOPS2 \\
HATS-33 & $ 7151.26648 $ & $    56.90 $ & $    11.80 $ & \nodata      & \nodata      & $   0.529 $ & CYCLOPS2 \\
HATS-33 & $ 7151.28183 $ & $    62.40 $ & $    14.80 $ & \nodata      & \nodata      & $   0.535 $ & CYCLOPS2 \\
HATS-33 & $ 7151.29714 $ & $    54.70 $ & $    12.20 $ & \nodata      & \nodata      & $   0.541 $ & CYCLOPS2 \\
HATS-33 & $ 7152.18422 $ & $    87.60 $ & $    10.40 $ & \nodata      & \nodata      & $   0.889 $ & CYCLOPS2 \\
HATS-33 & $ 7152.19954 $ & $    81.50 $ & $     8.60 $ & \nodata      & \nodata      & $   0.895 $ & CYCLOPS2 \\
HATS-33 & $ 7152.21486 $ & $    75.50 $ & $     7.40 $ & \nodata      & \nodata      & $   0.901 $ & CYCLOPS2 \\
HATS-33 & $ 7156.17139 $ & $   -38.60 $ & $    19.80 $ & \nodata      & \nodata      & $   0.453 $ & CYCLOPS2 \\
HATS-33 & $ 7156.18735 $ & $   -57.70 $ & $    17.20 $ & \nodata      & \nodata      & $   0.459 $ & CYCLOPS2 \\
HATS-33 & $ 7166.75718 $ & $   119.88 $ & $    10.00 $ & $   13.0 $ & $   14.0 $ & $   0.605 $ & FEROS \\
HATS-33 & $ 7179.83946 $ & $   219.96 $ & $    13.00 $ & $    5.0 $ & $   22.0 $ & $   0.736 $ & Coralie \\
HATS-33 & $ 7180.77062 $ & $  -154.04 $ & $    14.00 $ & $   53.0 $ & $   24.0 $ & $   0.102 $ & Coralie \\
HATS-33 & $ 7181.85831 $ & $    17.96 $ & $    14.00 $ & $   41.0 $ & $   22.0 $ & $   0.528 $ & Coralie \\
HATS-33 & $ 7182.81335 $ & $   123.96 $ & $    13.00 $ & $   34.0 $ & $   22.0 $ & $   0.903 $ & Coralie \\
HATS-33 & $ 7187.78052 $ & $   160.88 $ & $    10.00 $ & $    4.0 $ & $   12.0 $ & $   0.851 $ & FEROS \\
HATS-33 & $ 7187.79155 $ & $   132.88 $ & $    10.00 $ & $   12.0 $ & $   11.0 $ & $   0.855 $ & FEROS \\
HATS-33 & $ 7212.69884 $ & $    59.88 $ & $    12.00 $ & $  -63.0 $ & $   17.0 $ & $   0.625 $ & FEROS \\


==> data/HATS754-010_rvtable.tex <==
HATS-34 & $ 7181.90516 $ & $   156.41 $ & $    12.00 $ & $   16.0 $ & $   17.0 $ & $   0.737 $ & FEROS \\
HATS-34 & $ 7188.87902 $ & $   -25.59 $ & $    17.00 $ & $   16.0 $ & $   23.0 $ & $   0.048 $ & FEROS \\
HATS-34 & $ 7211.86173 $ & $    16.41 $ & $    14.00 $ & $  -20.0 $ & $   19.0 $ & $   0.960 $ & FEROS \\
HATS-34 & $ 7222.87045 $ & $  -161.59 $ & $    15.00 $ & $ -147.0 $ & $   20.0 $ & $   0.187 $ & FEROS \\
HATS-34 & $ 7223.79478 $ & $    85.41 $ & $    19.00 $ & $  -53.0 $ & $   25.0 $ & $   0.626 $ & FEROS \\
HATS-34 & $ 7224.81561 $ & $   -62.59 $ & $    18.00 $ & $  -10.0 $ & $   24.0 $ & $   0.111 $ & FEROS \\
HATS-34 & $ 7229.67888 $ & $   -83.59 $ & $    12.00 $ & $  -92.0 $ & $   16.0 $ & $   0.420 $ & FEROS \\


==> data/HATS779-003_rvtable.tex <==
HATS-35 & $ 6971.53689 $ & $   -83.38 $ & $    41.00 $ & $  -61.0 $ & $   29.0 $ & $   0.363 $ & Coralie \\
HATS-35 & $ 7119.91638 $ & $   116.74 $ & $    30.00 $ & $   99.0 $ & $   27.0 $ & $   0.846 $ & HARPS \\
HATS-35 & $ 7120.91245 $ & $  -119.26 $ & $    17.00 $ & $  -38.0 $ & $   18.0 $ & $   0.393 $ & HARPS \\
HATS-35 & $ 7179.85943 $\tablenotemark{d} & $   400.62 $ & $    44.00 $ & \nodata      & \nodata      & $   0.763 $ & Coralie \\
HATS-35 & $ 7180.79013 $ & $  -129.38 $ & $    53.00 $ & $ -999000.0 $ & $   38.0 $ & $   0.274 $ & Coralie \\
HATS-35 & $ 7181.87795 $ & $    87.62 $ & $    46.00 $ & $ -999000.0 $ & $   35.0 $ & $   0.872 $ & Coralie \\
HATS-35 & $ 7182.85998 $ & $  -153.38 $ & $    47.00 $ & $ -999000.0 $ & $   35.0 $ & $   0.411 $ & Coralie \\
HATS-35 & $ 7190.83382 $ & $   224.82 $ & $    22.00 $ & $   67.0 $ & $   14.0 $ & $   0.790 $ & FEROS \\
HATS-35 & $ 7191.72420 $ & $  -155.18 $ & $    20.00 $ & $   36.0 $ & $   14.0 $ & $   0.279 $ & FEROS \\
HATS-35 & $ 7192.65831 $ & $   209.82 $ & $    21.00 $ & $   58.0 $ & $   14.0 $ & $   0.792 $ & FEROS \\
HATS-35 & $ 7196.92836 $ & $  -124.18 $ & $    24.00 $ & $   60.0 $ & $   16.0 $ & $   0.137 $ & FEROS \\
HATS-35 & $ 7218.84882 $ & $  -112.18 $ & $    22.00 $ & $   91.0 $ & $   15.0 $ & $   0.174 $ & FEROS \\
HATS-35 & $ 7223.62885 $ & $   170.82 $ & $    25.00 $ & $   91.0 $ & $   17.0 $ & $   0.799 $ & FEROS \\
HATS-35 & $ 7224.52818 $ & $  -131.18 $ & $    22.00 $ & $   50.0 $ & $   15.0 $ & $   0.293 $ & FEROS \\
HATS-35 & $ 7226.86401 $ & $    14.82 $ & $    23.00 $ & $  -41.0 $ & $   15.0 $ & $   0.576 $ & FEROS \\
HATS-35 & $ 7229.85682 $ & $  -170.18 $ & $    23.00 $ & $    1.0 $ & $   15.0 $ & $   0.219 $ & FEROS \\
HATS-35 & $ 7230.84273 $ & $   178.82 $ & $    18.00 $ & $   35.0 $ & $   12.0 $ & $   0.761 $ & FEROS \\


==> newcommand_spec_multi_template.tex <==
%% GB's various newcommands for making editing easy for this specific paper

% This is the template version to be used for planets announced in a
% multi-planet paper. This file should be filled in separately for
% each planet in the paper. You should also find/replace the term
% xxxxx below with a unique identifier for each planet (e.g. xxxxA for
% the first one).  A version of this file should be saved with a
% unique name in the document directory for each planet, and all files
% should be processed into the newcommand_spec_multi.tex file using
% the scr/makenewcommand_spec_multi.sh script. This is done to allow
% you to reference planet information using commands like \hatcur{14}
% rather than \hatcurxxxxA. The newcommand_spec_multi.tex file so
% generated should not need to be edited or regenerated if changes are
% made to any of the planets parameters. Any changes should be made to
% the planet's own newcommand_spec.tex file.

% -------- Aliases specific to this paper/planet which should be edited -------

% The name of the host star and/or the planet:
\newcommand{\hatcurxxxxx}{HAT-P-14}
\newcommand{\hatcurbxxxxx}{HAT-P-14b}
\newcommand{\hatcurcxxxxx}{HAT-P-14c}

% The number used to index this system in the paper
\newcommand{\hatcurplanetnumxxxxx}{14}

%\newcommand{\hatcurCCraxxxxx}{\ensuremath{08^{\mathrm h}39^{\mathrm m}31.82^{\mathrm s}}}  % right ascension
%\newcommand{\hatcurCCdecxxxxx}{\ensuremath{+47^{\mathrm d}21^{\mathrm m}07.4^{\mathrm s}}} % declination

\newcommand{\hatcurRVgammaabsxxxxx}{\hatcurDSgamma{\hatcurplanetnumxxxxx}}                           % Absolute Gamma velocity

\newcommand{\hatcurRVgammarelxxxxx}{\hatcurRVgamma{\hatcurplanetnumxxxxx}}                           % Relative Gamma velocity. Typically that of the Keck RVs.

\newcommand{\hatcurCCtassvixxxxx}{\ensuremath{0.527\pm0.12}}                  % TASS V-I

\newcommand{\hatcurSMEversionxxxxx}{ii}                                       % Final SME version:i or ii?

% Isochrones used for this planet.
\newcommand{\hatcurisoshortxxxxx}{YY}
%\newcommand{\hatcurisoshortxxxxx}{Baraffe}
\newcommand{\hatcurisofullxxxxx}{Yonsei-Yale (YY)}
%\newcommand{\hatcurisofullxxxxx}{Baraffe}
\newcommand{\hatcurisocitexxxxx}{yi:2001}
%\newcommand{\hatcurisocitexxxxx}{baraffe:1998}

% Luminosity indicator used for this planet.
\newcommand{\hatcurlumindxxxxx}{\arstar}
%\newcommand{\hatcurlumindxxxxx}{Hip}s

% JHK filter type for the isochrone set used for this planet.
\newcommand{\hatcurjhkfilsetxxxxx}{ESO}
%\newcommand{\hatcurjhkfilsetxxxxx}{BB}
%\newcommand{\hatcurjhkfilsetxxxxx}{CIT}

% --------------------------------------------------------------------------
% The aliases below should not need editing, other than replaceing xxxxxx
% to whatever string.
% 
\newcommand{\hatcurSMEteffxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEiteff{\hatcurplanetnumxxxxx}}{\hatcurSMEiiteff{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEzfehxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEizfeh{\hatcurplanetnumxxxxx}}{\hatcurSMEiizfeh{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEzfehshortxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEizfehshort{\hatcurplanetnumxxxxx}}{\hatcurSMEiizfehshort{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEloggxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEilogg{\hatcurplanetnumxxxxx}}{\hatcurSMEiilogg{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEvsinxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEivsin{\hatcurplanetnumxxxxx}}{\hatcurSMEiivsin{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEvmacxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEivmac{\hatcurplanetnumxxxxx}}{\hatcurSMEiivmac{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEvmicxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEivmic{\hatcurplanetnumxxxxx}}{\hatcurSMEiivmic{\hatcurplanetnumxxxxx}}}

